PINT: Maximum-likelihood estimation of pulsar timing noise parameters

PINT is a pure-Python framework for high-precision pulsar timing developed on top of widely used and well-tested Python libraries, supporting both interactive and programmatic data analysis workflows. We present a new frequentist framework within PINT to characterize the single-pulsar noise processes present in pulsar timing datasets. This framework enables the parameter estimation for both uncorrelated and correlated noise processes as well as the model comparison between different timing and noise models in a computationally inexpensive way. We demonstrate the efficacy of the new framework by applying it to simulated datasets as well as a real dataset of PSR B1855+09. We also describe the new features implemented in PINT since it was first described in the literature.

==> components-table.tex <==
%% LyX 2.3.6 created this file.  For more info, see http://www.lyx.org/.
%% Do not edit unless you really know what you are doing.
% \documentclass[english]{article}
% \usepackage[T1]{fontenc}
% \usepackage[latin9]{inputenc}
% \usepackage{geometry}
% \geometry{verbose,tmargin=1.5cm,bmargin=1.5cm,lmargin=1.5cm,rmargin=1.5cm}
% \usepackage{textcomp}

% \makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
%% Because html converters don't know tabularnewline
% \providecommand{\tabularnewline}{\\}

% \makeatother

% \usepackage{babel}
% \begin{document}
% \begin{table}[]
%     % \centering
\begin{longtable}{|c|l|c|}
\hline 
\textbf{Component} & \textbf{Description} & \textbf{Reference}\tabularnewline
\hline 
\hline 
\multicolumn{3}{|l|}{\textbf{\emph{Pulsar rotation, rotational phase \& rotational irregularities}}}\tabularnewline
\hline 
\multicolumn{1}{|c|}{\texttt{Spindown}} & Taylor series representation of the pulsar rotation & Backer \& Hellings 1986\tabularnewline
\hline 
\texttt{PiecewiseSpindown §} & Piecewise-constant representation of pulsar rotation & \tabularnewline
\hline 
\texttt{Glitch} & Pulsar glitches & Hobbs et al 2006\tabularnewline
\hline 
\texttt{IFunc} & Piecewise or spline representation of rotational period & Deng et al 2012\tabularnewline
\hline 
\texttt{WaveX §} & Fourier series representation of achromatic red noise & Hobbs et al 2006\tabularnewline
 & (supersedes the deprecated \texttt{Wave} model) & \tabularnewline
\hline 
\texttt{PLRedNoise} & Fourier Gaussian process representation of achromatic red & Lentati et al 2016\tabularnewline
 & noise & \tabularnewline
\hline 
\texttt{AbsPhase} & Reference TOA with respect to which the rotational phase  & \tabularnewline
 & is measured & \tabularnewline
\hline 
\texttt{PhaseOffset §} & Overall phase offset between reference TOA and the physical & \tabularnewline
 & TOAs & \tabularnewline
\hline 
\texttt{PhaseJump} & Phase offsets between TOAs measured using different systems & Hobbs et al 2006\tabularnewline
\hline 
\multicolumn{3}{|l|}{\textbf{\emph{Binary system}}}\tabularnewline
\hline 
\texttt{BinaryBT} & Simple parametrized post-Keplerian binary model  & Blandford \& Teukolsky 1976\tabularnewline
 & (only Romer delay) & \tabularnewline
\hline 
\texttt{BinaryBTPiecewise §} & Similar to BinaryBT, but with piecewise-constant & \tabularnewline
 & orbital parameters & \tabularnewline
\hline 
\texttt{BinaryDD} & Parametrized post-Keplerian model (with Shapiro & Damour \& Deruelle 1986\tabularnewline
 & delay and Einstein delay) & \tabularnewline
\hline 
\texttt{BinaryDDGR §} & Similar to BinaryDD, but assumes General Relativity & \tabularnewline
\hline 
\texttt{BinaryDDH §} & Similar to BinaryDD, but uses a harmonic representation & Freire \& Wex 2010\tabularnewline
 & of Shapiro delay (for almost face-on systems) & Weisberg \& Huang 2016\tabularnewline
\hline 
\texttt{BinaryDDK} & Similar to BinaryDD, but includes Kopeikin delay & Damour \& Taylor 1992\tabularnewline
 &  & Kopeikin 1995, 1996\tabularnewline
\hline 
\texttt{BinaryDDS §} & Similar to BinaryDD, but uses an alternative representation & Kramer et al 2006\tabularnewline
 & of Shapiro delay (for almost edge-on orbits) & Rafikov \& Lai 2006\tabularnewline
\hline 
\texttt{BinaryELL1} & Binary model specialized for nearly circular orbits using & Lange et al 2001\tabularnewline
 & Laplace-Lagrange parameters & Zhu et al 2013\tabularnewline
 &  & Fiore et al 2023\tabularnewline
\hline 
\texttt{BinaryELL1H} & Similar to ELL1, but uses a harmonic representation of & Freire \& Wex 2010\tabularnewline
 & Shapiro delay (for almost face-on systems) & \tabularnewline
\hline 
\texttt{BinaryELL1k §} & Similar to ELL1, but includes an exact treatment of advance & Susobhanan et al 2018\tabularnewline
 & of periastron (for highly relativistic or tidally interacting  & \tabularnewline
 & binaries) & \tabularnewline
\hline 
\multicolumn{3}{|l|}{\textbf{Interstellar dispersion \& dispersion measure variations}}\tabularnewline
\hline 
\texttt{DispersionDM} & Taylor series representation of dispersion measure (DM) & Backer \& Hellings 1986\tabularnewline
\hline 
\texttt{DispersionDMX} & Piecewise-constant representation of DM variations & Arzoumanian et al 2015\tabularnewline
\hline 
\texttt{DMWaveX §} & Fourier series representation of DM variations & \tabularnewline
\hline 
\texttt{PLDMNoise §} & Fourier Gaussian process representation of DM  & Lentati et al. 2016\tabularnewline
 & variations & \tabularnewline
\hline 
\texttt{DispersionJump §} & Offsets between DMs measured using different systems & \tabularnewline
\hline 
\multicolumn{3}{|l|}{\textbf{\emph{Astrometry \& solar system delays}}}\tabularnewline
\hline 
\texttt{AstrometryEcliptic} & Astrometry in ecliptic coordinates & Edwards et al 2006\tabularnewline
\cline{1-2} \cline{2-2} 
\texttt{AstrometryEquatorial} & Astrometry in equatorial coordinates & \tabularnewline
\hline 
\texttt{SolarSystemShapiro} & Solar system Shapiro delay & Shapiro 1964\tabularnewline
\hline 
\multicolumn{3}{|l|}{\textbf{\emph{Solar wind}}}\tabularnewline
\hline 
\texttt{SolarWindDispersion §} & Solar wind model assuming a radial power-law relation for & Edwards et al 2006\tabularnewline
 & the electron density & You et al 2007, 2012\tabularnewline
\cline{1-2} \cline{2-2} 
\texttt{SolarWindDispersionX §} & Similar to SolarWindDispersion, but with a piecewise-constant & Madison et al 2019\tabularnewline
 & representation of the electron density. & Hazboun et al 2022\tabularnewline
\hline 
\multicolumn{3}{|l|}{\textbf{\emph{Troposphere}}}\tabularnewline
\hline 
\texttt{TroposphereDelay} & Tropospheric zenith delay and hydrostatic delay & Davis et al 1985\tabularnewline
 &  & Neill 1996\tabularnewline
\hline 
\multicolumn{3}{|l|}{\textbf{\emph{Time-uncorrelated noise}}}\tabularnewline
\hline 
\texttt{ScaleToaError} & Modifications to the measured TOA uncertainties   & Lentati et al. 2016\tabularnewline
\hline 
\texttt{ScaleDMError §} & Modifications to the measured wideband DM uncertainties & Alam et al 2021\tabularnewline
\hline 
\texttt{EcorrNoise} & Correlation between TOAs measured from the same  & Arzoumanian et al 2015\tabularnewline
 & observation & Johnson et al. 2023\tabularnewline
\hline 
\multicolumn{3}{|l|}{\textbf{\emph{Frequency-dependent profile evolution}}}\tabularnewline
\hline 
\texttt{FD} & Frequency-dependent profile evolution & Arzoumanian et al 2015\tabularnewline
\hline 
\texttt{FDJump §} & System and frequency-dependent profile evolution & \tabularnewline
\hline 
\caption{Caption}
\label{tab:my_label}
\end{longtable}
    
% \end{table}
% \end{document}

